Enhancing AUTOSAR-Based Firmware Over-the-Air Updates in the Automotive Industry with a Practical Implementation on a Steering System

The automotive industry is increasingly reliant on software to manage complex vehicle functionalities, making efficient and secure firmware updates essential. Traditional firmware update methods, requiring physical connections through On-Board Diagnostics (OBD) ports, are inconvenient, costly, and time-consuming. Firmware Over-the-Air (FOTA) technology offers a revolutionary solution by enabling wireless updates, reducing operational costs, and enhancing the user experience. This project aims to design and implement an advanced FOTA system tailored for modern vehicles, incorporating the AUTOSAR architecture for scalability and standardization, and utilizing delta updating to minimize firmware update sizes, thereby improving bandwidth efficiency and reducing flashing times. To ensure security, the system integrates the UDS 0x27 protocol for authentication and data integrity during the update process. Communication between Electronic Control Units (ECUs) is achieved using the CAN protocol, while the ESP8266 module and the master ECU communicate via SPI for data transfer. The system's architecture includes key components such as a bootloader, boot manager, and bootloader updater to facilitate seamless firmware updates. The functionality of the system is demonstrated through two applications: a blinking LED and a Lane Keeping Assist (LKA) system, showcasing its versatility in handling critical automotive features. This project represents a significant step forward in automotive technology, offering a user-centric, efficient, and secure solution for automotive firmware management.

==> chapters/appendices/app0A.tex <==
%
% file: localoperator.tex
% author: Victor Brena
% description: Briefly describes properties of the local operator.
%

\chapter{Appendix A}
\label{app:app01}

Begins an appendix









\
